Trace is the Next AutoDiff: Generative Optimization with Rich Feedback, Execution Traces, and LLMs

We study a class of optimization problems motivated by automating the design and update of AI systems like coding assistants, robots, and copilots. AutoDiff frameworks, like PyTorch, enable efficient end-to-end optimization of differentiable systems. However, general computational workflows can be non-differentiable and involve rich feedback (e.g. console output or user's responses), heterogeneous parameters (e.g. prompts, codes), and intricate objectives (beyond maximizing a score). We investigate end-to-end generative optimization -- using generative models such as LLMs within the optimizer for automatic updating of general computational workflows. We discover that workflow execution traces are akin to back-propagated gradients in AutoDiff and can provide key information to interpret feedback for efficient optimization. Formally, we frame a new mathematical setup, Optimization with Trace Oracle (OPTO). In OPTO, an optimizer receives an execution trace along with feedback on the computed output and updates parameters iteratively. We provide a Python library, Trace, that efficiently converts a workflow optimization problem into an OPTO instance using PyTorch-like syntax. Using Trace, we develop a general LLM-based generative optimizer called OptoPrime. In empirical studies, we find that OptoPrime is capable of first-order numerical optimization, prompt optimization, hyper-parameter tuning, robot controller design, code debugging, etc., and is often competitive with specialized optimizers for each domain. We envision Trace as an open research platform for devising novel generative optimizers and developing the next generation of interactive learning agents. Website: https://microsoft.github.io/Trace/.

==> background.tex <==















 








==> extra_codes.tex <==




    



\begin{lstlisting}[language=Python]

## Iteration 0 (initialization); Success: False
def controller(obs):
    """
    A feedback controller that computes the action based on the observation.

    Args:
        obs: (dict) The observation from the environment. Each key is a string (indicating a type of observation) and the value is a list of floats.
    Output:
        action: (list or nd.array) A 4-dimensional vector.
    """
    return [0, 0, 0, 0]


## Iteration 1; Success: False
def controller(obs):
    """
    A feedback controller that computes the action based on the observation.

    Args:
        obs: (dict) The observation from the environment. Each key is a string (indicating a type of observation) and the value is a list of floats.
    Output:
        action: (list or nd.array) A 4-dimensional vector.
    """
    hand_pos = obs['hand_pos']
    goal_pos = obs['goal_pos']
    action = [goal_pos[0] - hand_pos[0], goal_pos[1] - hand_pos[1], goal_pos[2] - hand_pos[2], 0]
    # Adjusting the last element of the action based on whether the hand is close enough to trigger grasping
    if abs(goal_pos[0] - hand_pos[0]) < 0.02 and abs(goal_pos[1] - hand_pos[1]) < 0.02 and abs(goal_pos[2] - hand_pos[2]) < 0.02:
        action[3] = 1 # Assuming action[3] = 1 triggers closing the gripper
    return action]    


## Iteration 7; Success: False
def controller(obs):
    """
    A feedback controller that computes the action based on the observation.

    Args:
        obs: (dict) The observation from the environment.
    Output:
        action: (list or nd.array) A 4-dimensional vector.
    """
    hand_pos = obs['hand_pos']
    puck_pos = obs['puck_pos']
    goal_pos = obs['goal_pos']
    gripper_open = 1 if obs['gripper_distance_apart'][0] > 0.5 else 0

    # Adjusting strategy to ensure the gripper closes when in the correct proximity of the puck
    if gripper_open and ((abs(hand_pos[0] - puck_pos[0]) < 0.05) and (abs(hand_pos[1] - puck_pos[1]) < 0.05) and (abs(hand_pos[2] - puck_pos[2]) < 0.05)):
        action = [0, 0, 0, 1]  # Close the gripper
    elif not gripper_open:
        # Adjust the direction towards the goal with respect to the current position and ensure the robot moves towards the goal position
        direction_to_goal = [goal_pos[0] - hand_pos[0], goal_pos[1] - hand_pos[1], goal_pos[2] - hand_pos[2]]
        normalize = lambda x: [i / max(abs(max(x, key=abs)), 1) for i in x]  # Normalize to restrict movement within a step
        action = normalize(direction_to_goal) + [0]  # Move towards the suggested pose once puck is grasped
    else:
        # Improve towards puck logic by adding normalized direction
        direction_to_puck = [puck_pos[0] - hand_pos[0], puck_pos[1] - hand_pos[1], puck_pos[2] - hand_pos[2]]
        normalize = lambda x: [i / max(abs(max(x, key=abs)), 1) for i in x]  # Normalize to restrict movement within a step
        action = normalize(direction_to_puck) + [0]  # Normalize to ensure it does not exceed max step size

    return action
\end{lstlisting}
    
\begin{lstlisting}[language=Python]

## Iteration 13; Success: True
def controller(obs):
    """
    A feedback controller that computes the action based on the observation.

    Args:
        obs: (dict) The observation from the environment.
    Output:
        action: (list or nd.array) A 4-dimensional vector.
    """
    hand_pos = obs['hand_pos']
    puck_pos = obs['puck_pos']
    goal_pos = obs['goal_pos']
    gripper_open = 1 if obs['gripper_distance_apart'][0] > 0.5 else 0

    normalize = lambda x: [i / max(abs(max(x, key=abs)), 1) for i in x]
    # Close the gripper when close to the puck and the gripper is open
    if gripper_open and ((abs(hand_pos[0] - puck_pos[0]) < 0.05) and (abs(hand_pos[1] - puck_pos[1]) < 0.05) and (abs(hand_pos[2] - puck_pos[2]) < 0.05)):
        action = [0, 0, 0, 1]  # Close the gripper
    elif not gripper_open and ((abs(hand_pos[0] - puck_pos[0]) < 0.1) and (abs(hand_pos[1] - puck_pos[1]) < 0.1) and (abs(hand_pos[2] - puck_pos[2]) < 0.1)):
        # When the puck is grasped, adjust direction towards the goal with improved precision and ensure successful pickup
        direction_to_goal = normalize([goal_pos[0] - hand_pos[0], goal_pos[1] - hand_pos[1], goal_pos[2] - hand_pos[2]])
        action = direction_to_goal + [1]  # Keep the gripper closed
    else:
        # Move towards the puck first if not carrying it
        direction_to_puck = normalize([puck_pos[0] - hand_pos[0], puck_pos[1] - hand_pos[1], puck_pos[2] - hand_pos[2]])
        action = direction_to_puck + [0]  # Open the gripper to prepare for grasping

    return action



\end{lstlisting}


==> usage.tex <==
\section{Example of \trace and \algo in action}
\label{sec:usage}

\adith{\trace is a more general tool than backpropagation. It can be used to describe the joint optimization of codes, strings and numbers as we will see in the following example of optimizing chained functions.}

Consider an example workflow of an AI agent for the game of Battleship (Figure~\ref{fig:overall_pipeline}, left). 
The agent must implement two underlying functions of the \verb|place_shot| function: \verb|reason| (line $9$) and \verb|act| (line $16$) to react intelligently to different board positions. 
The Battleship environment provides feedback by executing the \verb|place_shot| function on a game board. 
These could be e.g. syntax errors in a candidate \verb|place_shot| implementation or semantic errors when executing them (such as \texttt{index out of bounds}) or \texttt{Hit/Miss} feedback. 
The goal of an optimizer is to use the observed feedbacks to improve the \verb|place_shot| heuristic.

Imagine how a programmer might modify the \verb|place_shot| heuristic using feedbacks. When they observe a stack trace caused by syntax errors (i.e., rich feedback), they can pinpoint where \verb|place_shot| should be modified because they can see the execution inside the function. They know that \verb|place_shot| invokes \verb|reason| and \verb|act|, and they know how the input and output are used.
Our \trace framework achieves this same effect without introducing additional complexity to the Python code. 
\trace monitors the execution of a workflow, and records all usages of any parameters (declared using \verb|trainable=True| on line $8$) to construct a directed acyclic graph representing the computation (\adith{foreshadow Figure~\ref{fig:optimization}}).
In Figure~\ref{fig:battleship-learning}, we show that even with verbal feedback, we can gradually learn functions of increasingly complex heuristics. 
































